Natural Language Processing Methods for Symbolic Music Generation and Information Retrieval: a Survey

Several adaptations of Transformers models have been developed in various domains since its breakthrough in Natural Language Processing (NLP). This trend has spread into the field of Music Information Retrieval (MIR), including studies processing music data. However, the practice of leveraging NLP tools for symbolic music data is not novel in MIR. Music has been frequently compared to language, as they share several similarities, including sequential representations of text and music. These analogies are also reflected through similar tasks in MIR and NLP. This survey reviews NLP methods applied to symbolic music generation and information retrieval studies following two axes. We first propose an overview of representations of symbolic music adapted from natural language sequential representations. Such representations are designed by considering the specificities of symbolic music. These representations are then processed by models. Such models, possibly originally developed for text and adapted for symbolic music, are trained on various tasks. We describe these models, in particular deep learning models, through different prisms, highlighting music-specialized mechanisms. We finally present a discussion surrounding the effective use of NLP tools for symbolic music data. This includes technical issues regarding NLP methods and fundamental differences between text and music, which may open several doors for further research into more effectively adapting NLP tools to symbolic MIR.

==> secsub-intro-music_linguistic.tex <==
\subsection{Music seen as a linguistic system}
\label{sec:intro_music_language}
Beyond computer science studies, parallels between music and natural language appear at multiple levels, encompassing their role as communication tools as well as their inner structures.


\input{figs/fig_music_text_segmentations}

Music and text are first comparable at a low level, as they share 
similarities in their constitutive elements.
Text representations and symbolic music representations are both semiotic systems~\cite{chomsky1979human}: text is often based on characters, and written music can be retranscribed with scores using standard notation or non-western notation systems, such as numbered notation, or instrument-specific notations such as tablatures.
In other words, they consist of arrangements of symbols, with both systems being based on various \textit{signs}.


They can be represented as sequences of elements that can be segmented or grouped at different levels. 
Text can be segmented into characters, syntactic phrases and sentences, in the same way as music 
can typically be segmented into temporal units such as notes, motifs, musical phrases, or sections~\cite{lerdahl2013musical},
as represented in Figure~\ref{fig:music_text_segmentations}.




At a higher level, 
multiple models of musical syntaxes have been proposed~\cite{bernstein1976unanswered,bod2002unified,hirata2022formal}
in order to propose a similar concept with linguistic grammar or syntax.
When formal and natural languages employ tree structures to depict syntax or grammar,
music, on the other hand, relies on intrinsic musical concepts such as tension and relaxation~\cite{lerdahl1996generative} or harmony~\cite{rohrmeier2011towards} to construct similar tree-like representations.
These grammatical or syntactic rules lead to expectancy in both language and music~\cite{jackendoff2009parallels,pearce2018statistical}, inducing similar cognitive reactions for the interlocutor or the listener when they are being transgressed in both language~\cite{pulvermuller2007grammar} and music~\cite{besson2001comparison,hoch2008musique}. 
Over the years, research in the field of cognitive science has provided insights into both music and language.
For example, high pitch has been shown to be associated with a fear response~\cite{huron2015cues}: such common cognitive reactions are similar in both music and speech.



Finally, beyond its formal description, music also shares similarities with text from a human perspective. 
Music is often considered as having similar origins with language~\cite{wallin2001origins}. %
Both are specific to human species and are learned through imitation and can both be perceived as elements unfolding in time~\cite{zbikowski2009music,wallin2001origins}, as well as being deployed under two modalities: an annotated form (text, sheet music) and an auditory form (speech, musical performance)~\cite{cross2005music,fornas1997text}.
Therefore, music and language are often considered arts since they both require imagination and expressiveness~\cite{clark1982music}.
Hence, when talking about music, various expressions employ language-related terms, such as ``call-and-response'' to denote responsorial writing or melodic lines shared by two or more instruments, or ``musical discourse'' that can denote the high-level structure of a piece.
Lower-level musical structures or objects are also referred to using natural language terms, such as ``musical phrases'' or ``punctuation''.



However, major distinctions and particularities still persist between music and text.
Among others, polyphony, where multiple parts can occur simultaneously, is a characteristic of music that does not have any equivalent in text. 
Beyond this vertical axis describing harmony, another significant difference between text and music lies in the temporal dimension. 
In music, events must occur at precise timings, following specific rhythms, which contrasts with text where such a rigorous time grid does not exist.
Finally, at a much lower level, unlike textual Latin characters, musical notes are multimodal, characterized by multiple aspects, such as their pitch, duration, dynamics, and more. 
Addressing such issues specific to music has led to the development of various approaches to represent and approximate music as a sequence of elements. 

Although these differences between text and music, 
which will be further discussed in Section~\ref{sec:discussion}, 
MIR studies have leveraged the similarities between text and music to adapt and apply NLP methods on symbolic musical data.



==> secsub-intro-tasks.tex <==
\subsection{Symbolic MIR and NLP tasks: similarities and specificities}
\label{sec:tasks}


Beyond the similarities between text and symbolic music data, the Natural Language Processing and Music Information Retrieval research fields are also related in terms of addressed tasks.
Parallels can be drawn across multiple tasks in both fields.
MIR tasks presented in the following are not strictly derived or influenced by NLP, but are so closely related that MIR studies have been prompted to adapt NLP models and representations for symbolic music. 
Such NLP and MIR tasks can be grouped into two categories based on the type of data on which the model is trained: \textit{labeled} or \textit{unlabeled} data, depending on whether the task solution relies, or not, on the availability of labels for a set of data.
From a technical point of view, labeled data are handled by \textit{supervised learning} tasks, in contrast with \textit{unsupervised} or \textit{self-supervised} learning tasks which handle unlabeled data. 






\subsubsection{Tasks on labeled data}
Such tasks rely on datasets of labeled text or symbolic music, with labels typically derived from human annotations or possibly automated analysis.
In both MIR and NLP, such data labeling can either take place at a global level, where a label describes an entire text document or music piece, or at a local level, where labels describe specific parts or sections of the document.

Text and music can be classified following various characteristics, with one label describing a whole textual document or music piece.
Music composer classification~\cite{pollastri2001classification} or text authorship attribution~\cite{stamatatos2009survey} are common downstream classification tasks. Cultural origin classification tasks are also widespread with folk song classification~\cite{hillewaere2009global} can be analogous to language detection in multilingual text~\cite{jauhiainen2019automatic}.
Beyond these objective tasks, text style and music genre classification are also often considered as baseline tasks.
Model performances on music genre~\cite{correa2016classification} or text style~\cite{kessler1997automatic} classification are often dependant on the considered data as boundaries between music style as jazz and blues, or text genres as editoral or non-fictional tasks are often non-consensual.
Finally, the availability of text and music datasets with emotions~\cite{hung2021emopia} or sentiment~\cite{wankhade2022survey} annotations, while being intrinsically subjective, enables the design of models dedicated to the prediction of these features.



Text and symbolic music are constructed with high level structures, such as paragraphs or musical phrases (Figure~\ref{fig:music_text_segmentations}), which naturally leads to a variety of segmentation tasks in both domains.
Multiple studies have therefore tackled segmentation tasks in both text in music.
Music segmentation includes musical phrase retrieval~\cite{guan2018melodic}, and at a higher level, musical form segmentation including sonata form~\cite{allegraud2019learning} or fugues~\cite{giraud2015computational}.
On the textual side, such segmentation tasks can occur at a semantic level with topic segmentation~\cite{ponte1997text}, discourse parsing~\cite{lin2019unified} or at a lower level with sentence segmentation in languages such as Chinese~\cite{huang2010classical} where the absence of punctuation can make this task nontrivial.
Such tasks can also be modeled based on an unsupervised training paradigm, in which models process and learn from unlabeled data, instead of relying on labeled datasets containing expert annotations.

\subsubsection{Tasks on unlabeled data}
Unlabeled music datasets~\cite{morreale2023data,dong2020muspy} and text datasets are abundant as they consist of raw symbolic music or text.
Such datasets support multiple NLP and MIR tasks that follow two main learning paradigms: \textit{unsupervised} learning and \textit{self-supervised} learning.
Unsupervised learning involves training a model on data without labeled outcomes, aiming to discover inherent patterns or structures within the data. 
Self-supervised learning is a specific type of unsupervised learning where the model creates its own labels from the input data, often by predicting parts of the input itself, enabling it to learn representations and patterns without external annotations.


Unsupervised learning tasks, present both in MIR and NLP, rely on a notion of musical and textual similarity.
Music similarity can be examined at the level of musical segments for unsupervised melodic phrase segmentation purposes~\cite{janssen2017finding}, or at a higher level, as seen in the genre classification task, which is considered as a clustering problem~\cite{cilibrasi2004clustering}.
Similarly, text studies also focus on such similarity retrieval tasks that occur at multiple levels, from word clustering~\cite{xu2015short} to full document clustering~\cite{blei2003latent,rafi2013improved}.



Among self-supervised learning tasks, generative tasks are the most studied tasks in both NLP and MIR.
Symbolic music generation can involve different musical objects at different scales~\cite{huang2020ai}: the structure of the piece, harmony and chords, notes, etc. with various generation conditions~\cite{ji2023survey}.
In NLP, where the generated content is always textual data, multiple constraints and purposes define these generative tasks. %
\url{https://www.innerdoc.com/periodic-table-of-nlp-tasks/}}.
The generated content in NLP and MIR generative tasks can be conditioned by local constraints (\ie the neighboring context) or globally on the entire sequence.

Local constraints can be placed in various positions to control the generated content.
Infilling tasks refer to generating content in between two constraints defined by a starting and an ending chunk of text or music. Such infilling tasks are well-explored in MIR~\cite{chang2021variable,guo2022musiac} and in NLP~\cite{zhu2019text,donahue2020enabling}.
Instead of filling in the blanks in the middle of a document or a piece, a unique constraint can be placed at the beginning, leading to music priming~\cite{huang2018music} or text continuation~\cite{radford2019language}.
Such constraint can also be global and of another nature than text or music, aiming at controlling the entire generated content.
Style transfer consists in generating textual or musical elements starting from an initial document or piece and transforming it into another style, while keeping a similar content. These styles can refer to musical genre~\cite{ding2022steelygan,wu2023musemorphose} or language high-level elements such as formality or toxicity~\cite{jin2022deep}.
More recently, text-conditioned generation has become more and more popular for the general public, including chatbot dialog\footnote{\url{https://chat.openai.com}} in the NLP field, but also text-conditioned symbolic music generation with text-to-MIDI~\cite{lu2023musecoco}.













Despite of all these common tasks between NLP and symbolic MIR, these two fields still present numerous specific tasks that lack equivalents in the other, as depicted in Figure~\ref{fig:survey_overview}. 
Examples include named-entity recognition, coreference resolution or question answering in text, and key detection, chord progression generation or harmonization in music. 
These tasks specific to each field also reflect the inherent differences between these two types of data. 
Some concepts are inherent to text, such as semantics, whereas musical concepts do not find any analogous notion in text, like event simultaneity leading to harmony.

